Mapping with Reflection -- Detection and Utilization of Reflection in 3D Lidar Scans

This paper presents a method to detect reflection of 3D light detection and ranging (Lidar) scans and uses it to classify the points and also map objects outside the line of sight. Our software uses several approaches to analyze the point cloud, including intensity peak detection, dual return detection, plane fitting, and finding the boundaries. These approaches can classify the point cloud and detect the reflection in it. By mirroring the reflection points on the detected window pane and adding classification labels on the points, we can improve the map quality in a Simultaneous Localization and Mapping (SLAM) framework. Experiments using real scan data and ground truth data showcase the effectiveness of our method.

==> References/references.tex <==
% !TEX root = ../Thesis_template.tex
\addcontentsline{toc}{chapter}{\protect \textbf{References}}
\nocite{*}
\renewcommand{\bibname}{References}           % change default name Bibliography to References
\printbibliography

%\begin{figure}
%\setboolean{@twoside}{false}
% Uncomment the follow line to show the survey
%\end{figure}

%\begin{figure}
 %\centering 
 %\includegraphics{Appendix2/gbhri3_format.pdf}
%\end{figure}

